Interpreting Deep Learning Model Using Rule-based Method

Deep learning models are favored in many research and industry areas and have reached the accuracy of approximating or even surpassing human level. However they've long been considered by researchers as black-box models for their complicated nonlinear property. In this paper, we propose a multi-level decision framework to provide comprehensive interpretation for the deep neural network model. In this multi-level decision framework, by fitting decision trees for each neuron and aggregate them together, a multi-level decision structure (MLD) is constructed at first, which can approximate the performance of the target neural network model with high efficiency and high fidelity. In terms of local explanation for sample, two algorithms are proposed based on MLD structure: forward decision generation algorithm for providing sample decisions, and backward rule induction algorithm for extracting sample rule-mapping recursively. For global explanation, frequency-based and out-of-bag based methods are proposed to extract important features in the neural network decision. Furthermore, experiments on the MNIST and National Free Pre-Pregnancy Check-up (NFPC) dataset are carried out to demonstrate the effectiveness and interpretability of MLD framework. In the evaluation process, both functionally-grounded and human-grounded methods are used to ensure credibility.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	samples/sample-manuscript.tex \
	samples/sample-acmsmall.tex \
	samples/sample-acmlarge.tex \
	samples/sample-acmtog.tex \
	samples/sample-sigconf.tex \
	samples/sample-authordraft.tex \
	samples/sample-xelatex.tex \
	samples/sample-sigplan.tex \
	samples/sample-sigchi.tex \
	samples/sample-sigchi-a.tex


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

samples/%: %
	cp $^ samples

samples/sample-acmsmall.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmsmall]{acmart}/' $< > $@

samples/sample-acmlarge.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmlarge,screen]{acmart}/' $< > $@

samples/sample-acmtog.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[acmtog]{acmart}/' $<   > $@

samples/sample-sigconf.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-authordraft.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigconf,authordraft]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-xelatex.tex: samples/sample-sigconf.tex
	cp $< $@

samples/sample-sigplan.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigplan,screen]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi]{acmart}/' $< | sed 's/^%%//'  > $@

samples/sample-sigchi-a.tex: samples/sample-manuscript.tex
	sed 's/documentclass\[manuscript,screen\]{acmart}/documentclass[sigchi-a]{acmart}/' $< | \
	sed 's/begin{figure}\[h\]/begin{marginfigure}/' | \
	sed 's/end{figure}/end{marginfigure}/' | \
	sed 's/begin{table}/begin{margintable}/' | \
	sed 's/end{table}/end{margintable}/'   > $@


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex $(notdir $<)
	cd $(dir $@) && pdflatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex $(notdir $<)
	cd $(dir $@) && xelatex $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut

distclean: clean


#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf samples/sample-*.pdf *.cls *.bst


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.

Version 1.57    Change of \baselinestretch now produces an error
		Booktabs is now always loaded
		Added option `balance' to balance last page in two-column mode
		E-mail is no longer split in addresses
		New samples (Stephen Spencer)

==> others.tex <==
%~\cite{madry2017pgd,rony2019ddn}. The adversarial training methods use adversarial examples generated by PGD and DDN to train the classifier, and then generate new adversarial examples to attacked the adversarially trained classifier. Through iterating the training and attack process, the classifier is expected to converge to a robust state. Compared with our detector-rectifier framework, adversarial training is a very time and computational resource consuming approach.

%For the end-to-end attacks, we have three threat models: grey-box, black-box, and white-box. In grey-box attacks, attackers have knowledge of the network parameters and structures of the classifier but are not aware that the classifier is under the protection of some defensive mechanism. In black-box attacks, attackers have no access to the classifier and does not know if the model is under protection. In white-box attacks, attackers are aware that the target model is under the protection of a specific defense, and have full access to the target model and the defensive scheme.




 For ORG and IG, the success rates even reach to 98\%. Nevertheless, 
%We compared the attack success rate of the transferable examples to the four sub-detectors and \dname. In order to ensure the transferable examples can not only attack the detectors but also can attack the final classifier, the detector-targeted attackers perturb the adversarial examples targeted to the classifier $F$ to generate the detector-targeted adversarial examples. In each row of Tab.~\ref{tab:robustness}, we lists the attack success rate of a given type of transferable examples to different sub-detectors and \name.

its corresponding sub-detector can not be adversarially attacked and we did not include it in the.


that are generated to different targeted detectors.

Here, we generate transferable examples targeted to VG-based, GBP-based, IG-based and ORG-based sub-detectors.


In white-box scenarios, we can train an model to



threat, we can train an attacker that can generate adversarial examples to fool our detector.



%our model The white-box attack is a serious threat to neural network-based detector is detector-targeted adversarial attacks, \ie training an attacker that can generate adversarial examples to fool our detector.

\dname was trained by adversarial examples that were generated by

of all eight types of attackers. Oppositely, unvaccinated training means \dname was trained by adversarial examples of a subset of the eight types of attackers.



A vaccinated trained model has seen all types of attacks in the training step, while some types of attacks

A vaccinated trained model

This is very like letting immune systems generate antibodies by injecting the vaccine, so we call this setup as vaccinated training.



\paratitle{Performance of Vaccinated Training.} Table~\ref{tab:vaccinated} gives the performance evaluation of \dname with a {\em Vaccinated Training} setup. Here, we adopted eight types of attackers to fool \name and the baselines, and meanwhile, the training examples of \name were also generated by the same eight types of attackers. In other words, the model has seen all types of attack examples in the training step. This is very like letting immune systems generate antibodies by injecting the vaccine, so we call this setup as vaccinated training.

a set of training samples and then use these adversarial examples (mixed with original training samples) to train our detector. Next, we use the same attackers to generate adversarial examples and mix them with original test samples as a test set.

 the Area Under the Curve (AUC) of the Receiver Operating Characteristic (ROC) curve as a performance metric to measure the



We report the performance of adversarial/original classification over the test set to evaluate the detector. As adversarial examples detection is a binary classification, we adopt the Area Under the Curve (AUC) of the Receiver Operating Characteristic (ROC) curve as a performance metric.

of example's network middle layer outputs to measure different between adversarial and benign examples.


%distribution of

 is also a thresholds based detection method. The criterion is Mahalanobis distance-based score which is the weighted average consisting of Mahalanobis distance between test sample and the closest empirical class-conditional Gaussian distribution from different network layers.


It constructs two hand-crafted features to express an sample, and defined two rules to detect adversarial examples. The rules paradoxical nature of benign images

rules to decide

is a thresholds based detection method. The criterions utilize the seemingly paradoxical nature of benign images, which is being close to the decision boundary as well as having low density directions leading towards the boundaries. Performance of TWS against especially white-box attack has been proven to be promising.


% is a neural net based statistical test. The test statistics utilizes PixelCNN, which captures the inherent property of clean image distribution, to verify if the input is also drawn from the same distribution.


%Two of the baselines are hand-crafted features-based, which are



And the one is a

two state-of-the-art hand-crafted features-based detectors and a neural network-based detector, which are


$\bullet$ {\em PixelDefend (PD)}~\cite{song2017pixeldefend} is a neural net based statistical test. The test statistics utilizes PixelCNN, which captures the inherent property of clean image distribution, to verify if the input is also drawn from the same distribution.

% Table generated by Excel2LaTeX from sheet '¶Ëµ½¶Ë'
\begin{table*}[t] \footnotesize
  \centering
  \caption{Classification accuracy of \name and the baselines.}
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{19}{c}{Grey-Box} \\
    \midrule
      & \multicolumn{6}{c|}{Fashion-MNIST} & \multicolumn{6}{c|}{CIFAR-10} & \multicolumn{6}{c}{ImageNet} \\
    \midrule
      & Our & PD & DDN & PGD & TVM & F & Our & PD & DDN & PGD & TVM & F & Our & PD & DDN & PGD & TVM & F \\
    \midrule
    Clean & 0.90 & 0.90 & 0.86 & 0.84 & 0.67 & \textbf{0.92} & 0.82 & 0.79 & 0.75 & 0.64 & 0.35 & \textbf{0.86} & 0.89 &   & 0.78 & 0.72 & 0.75 & \textbf{0.95} \\ \hline
    FGSM & \textbf{0.84} & 0.75 & 0.82 & 0.82 & 0.49 & 0.56 & 0.48 & 0.36 & \textbf{0.55} & 0.43 & 0.29 & 0.24 & \textbf{0.60} &   & 0.49 & 0.47 & 0.36 & 0.44 \\
    PGD-U & \textbf{0.79} & 0.64 & 0.80 & 0.81 & 0.57 & 0.27 & \textbf{0.41} & 0.30 & 0.37 & 0.35 & 0.32 & 0.08 & \textbf{0.75} &   & 0.38 & 0.47 & 0.66 & 0.02 \\
    PGD-T & \textbf{0.89} & 0.86 & 0.84 & 0.87 & 0.53 & 0.66 & 0.60 & \textbf{0.62} & 0.33 & 0.48 & 0.32 & 0.05 & 0.70 &   & 0.29 & 0.51 & \textbf{0.73} & 0.00 \\ \hline
    Dfool & 0.87 & \textbf{0.88} & 0.26 & 0.76 & 0.65 & 0.00 & 0.68 & \textbf{0.71} & 0.19 & 0.29 & 0.34 & 0.00 & 0.71 &   & 0.37 & 0.35 & \textbf{0.75} & 0.01 \\
    CW-U & 0.86 & \textbf{0.88} & 0.70 & 0.73 & 0.66 & 0.00 & \textbf{0.74} & 0.73 & 0.70 & 0.63 & 0.34 & 0.00 & 0.71 &   & 0.50 & 0.53 & \textbf{0.74} & 0.00 \\
    CW-T & \textbf{0.86} & \textbf{0.86} & 0.72 & 0.53 & 0.65 & 0.00 & 0.64 & \textbf{0.75} & 0.45 & 0.46 & 0.33 & 0.00 & \textbf{0.79} &   & 0.40 & 0.39 & 0.75 & 0.00 \\
    DDN-U & \textbf{0.90} & 0.89 & 0.74 & 0.76 & 0.66 & 0.00 & 0.65 & \textbf{0.74} & 0.66 & 0.52 & 0.34 & 0.00 & \textbf{0.76} &   & 0.56 & 0.44 & 0.75 & 0.03 \\
    DDN-T & \textbf{0.90} & 0.89 & 0.59 & 0.64 & 0.65 & 0.00 & 0.71 & \textbf{0.75} & 0.53 & 0.43 & 0.34 & 0.00 & 0.79 &   & 0.50 & 0.39 &   & 0.00 \\
    \midrule
    \multicolumn{19}{c}{Black-Box} \\
    \midrule
      & \multicolumn{6}{c|}{Fashion-MNIST} & \multicolumn{6}{c|}{CIFAR-10} & \multicolumn{6}{c}{ImageNet} \\
    \midrule
      & Our & PD & DDN & PGD & TVM & F & Our & PD & DDN & PGD & TVM & F & Our & PD & DDN & PGD & TVM & F \\
    \midrule
    Clean & 0.90 & 0.90 & 0.86 & 0.84 & 0.67 & \textbf{0.92} & 0.82 & 0.79 & 0.75 & 0.64 & 0.35 & \textbf{0.86} & 0.89 &   & 0.78 & 0.72 & 0.75 & \textbf{0.95} \\ \hline
    FGSM & 0.71 & \textbf{0.72} & 0.68 & 0.71 & 0.46 & 0.50 & 0.31 & 0.27 & \textbf{0.41} & \textbf{0.41} & 0.31 & 0.50 & \textbf{0.60} &   & 0.51 & 0.48 & 0.54 & 0.50 \\
    PGD-U & 0.78 & 0.80 & 0.77 & \textbf{0.82} & 0.48 & 0.50 & 0.55 & \textbf{0.70} & 0.68 & 0.58 & 0.31 & 0.50 & \textbf{0.63} &   & 0.58 & 0.50 & 0.51 & 0.50 \\
    PGD-T & 0.79 & 0.78 & 0.74 & \textbf{0.81} & 0.43 & 0.50 & 0.63 & \textbf{0.73} & 0.70 & 0.59 & 0.30 & 0.50 & \textbf{0.65} &   & 0.55 & 0.49 & 0.50 & 0.50 \\ \hline
    Dfool & \textbf{0.87} & 0.86 & 0.84 & \textbf{0.87} & 0.48 & 0.50 & \textbf{0.78} & 0.76 & 0.71 & 0.61 & 0.29 & 0.50 & \textbf{0.67} &   & 0.58 & 0.51 &   & 0.50 \\
    CW-U & \textbf{0.88} & 0.87 & 0.84 & 0.87 & 0.48 & 0.50 & \textbf{0.78} & 0.75 & 0.71 & 0.61 & 0.30 & 0.50 & \textbf{0.65} &   & 0.51 & 0.51 & 0.46 & 0.50 \\
    CW-T & 0.86 & \textbf{0.87} & 0.84 & \textbf{0.87} & 0.53 & 0.50 & \textbf{0.77} & 0.75 & 0.71 & 0.60 & 0.29 & 0.50 & \textbf{0.67} &   & 0.56 & 0.51 & 0.44 & 0.50 \\
    DDN-U & \textbf{0.88} & 0.87 & 0.84 & 0.87 & 0.50 & 0.50 & \textbf{0.77} & 0.76 & 0.72 & 0.61 & 0.30 & 0.50 & \textbf{0.67} &   & 0.57 & 0.50 & 0.45 & 0.50 \\
    DDN-T & \textbf{0.88} & 0.87 & 0.84 & 0.87 & 0.49 & 0.50 & \textbf{0.77} & 0.74 & 0.71 & 0.60 & 0.28 & 0.50 & \textbf{0.68} &   & 0.53 & 0.46 & 0.41 & 0.50 \\
    \bottomrule
    \end{tabular}%
  \label{tab:end2end}%
\end{table*}%

% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[t]\small
  \centering
  \caption{Classification Accuracy of \name and Baselines}
    \begin{tabular}{l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r|r}
    \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} & \multicolumn{1}{r}{} &  \\
    \midrule
    \multicolumn{19}{c}{Grey-Box} \\
    \midrule
          & \multicolumn{6}{c|}{Fashion-MNIST}            & \multicolumn{6}{c|}{CIFAR-10}                 & \multicolumn{6}{c}{ImageNet} \\
    \midrule
          & \multicolumn{1}{l|}{Our} & \multicolumn{1}{l|}{PD} & \multicolumn{1}{l|}{DDN} & \multicolumn{1}{l|}{PGD} & \multicolumn{1}{l|}{TVM} & \multicolumn{1}{l|}{F} & \multicolumn{1}{l|}{Our} & \multicolumn{1}{l|}{PD} & \multicolumn{1}{l|}{DDN} & \multicolumn{1}{l|}{PGD} & \multicolumn{1}{l|}{TVM} & \multicolumn{1}{l|}{F} & \multicolumn{1}{l|}{Our} & \multicolumn{1}{l|}{PD} & \multicolumn{1}{l|}{DDN} & \multicolumn{1}{l|}{PGD} & \multicolumn{1}{l|}{TVM} & \multicolumn{1}{l}{F} \\
    \midrule
    Clean &   0.99    &    0.99   &    0.99   &    0.99   &    0.99   &    0.99   &     0.99  &   0.99    &    0.99   &    0.99   &    0.99   &    0.99   &    0.99   &   0.99    &    0.99   &      0.99 &   0.99    & 0.99 \\
    FGSM  &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    PGD-T &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    PGD-U &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Dfool &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    CW-T  &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    CW-U  &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    DDN-T &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    DDN-U &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \midrule
    \multicolumn{19}{c}{Black-Box} \\
    \midrule
          & \multicolumn{6}{c|}{Fashion-MNIST}            & \multicolumn{6}{c|}{CIFAR-10}                 & \multicolumn{6}{c}{ImageNet} \\
    \midrule
          & \multicolumn{1}{l|}{Our} & \multicolumn{1}{l|}{PD} & \multicolumn{1}{l|}{DDN} & \multicolumn{1}{l|}{PGD} & \multicolumn{1}{l|}{TVM} & \multicolumn{1}{l|}{F} & \multicolumn{1}{l|}{Our} & \multicolumn{1}{l|}{PD} & \multicolumn{1}{l|}{DDN} & \multicolumn{1}{l|}{PGD} & \multicolumn{1}{l|}{TVM} & \multicolumn{1}{l|}{F} & \multicolumn{1}{l|}{Our} & \multicolumn{1}{l|}{PD} & \multicolumn{1}{l|}{DDN} & \multicolumn{1}{l|}{PGD} & \multicolumn{1}{l|}{TVM} & \multicolumn{1}{l}{F} \\
    \midrule
    Clean &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    FGSM  &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    PGD-T &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    PGD-U &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    Dfool &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    CW-T  &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    CW-U  &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    DDN-T &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    DDN-U &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &       &  \\
    \bottomrule
    \end{tabular}%
  \label{tab:end2end}%
\end{table*}%


\begin{table*}[t]\footnotesize
  \centering
  \caption{Classification Accuracy of \name}
    \begin{tabular}{l|c|c|c|c|c|c|c|c|c|c|l|c|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{11}{c|}{Grey-Box}            & \multicolumn{9}{c}{Black-Box} \\
    \midrule
    --  & \multicolumn{5}{c|}{Fashion-MNIST} & \multicolumn{5}{c|}{CIFAR-10} &  -- & \multicolumn{4}{c|}{Fashion-MNIST} & \multicolumn{4}{c}{CIFAR-10} \\
    \midrule
    --  & Our & PD & DDN$_a$ & PGD$_a$ & $F$ & Our & PD & DDN$_a$ & PGD$_a$ & $F$ & --  & Our & PD & DDN$_a$ & PGD$_a$ & Our & PD & DDN$_a$ & PGD$_a$ \\
    \midrule
    Clean & 0.90 & 0.90 & 0.86 & 0.84 & \textbf{0.92} & 0.82 & 0.79 & 0.75 & 0.64 & \textbf{0.86} &  Clean & 0.90 & 0.90 & 0.86 & 0.84 & 0.82 & 0.79 & 0.75 & 0.64 \\ \hline
    FGSM & \textbf{0.84} & 0.75 & 0.82 & 0.82 & 0.56 & 0.48 & 0.36 & \textbf{0.55} & 0.43 & 0.24 &  FGSM & 0.71 & 0.72 & 0.68 & 0.71 & 0.31 & 0.27 & \textbf{0.41} & \textbf{0.41} \\
    PGD-T & \textbf{0.80} & 0.64 & 0.80 & 0.81 & 0.27 & \textbf{0.41} & 0.30 & 0.37 & 0.35 & 0.08 &  PGD-U & 0.78 & 0.80 & 0.77 & \textbf{0.82} & 0.55 & \textbf{0.70} & 0.68 & 0.58 \\
    PGD-U & \textbf{0.89} & 0.86 & 0.84 & 0.87 & 0.66 & 0.60 & \textbf{0.62} & 0.33 & 0.48 & 0.05 &  PGD-T & 0.79 & 0.78 & 0.74 & 0.81 & 0.63 & \textbf{0.73} & 0.70 & 0.59 \\ \hline
    DFool & \textbf{0.88} & 0.87 & 0.26 & 0.76 & 0.00 & 0.68 & \textbf{0.71} & 0.19 & 0.29 & 0.00 &  DFool & 0.87 & 0.86 & 0.84 & 0.87 & 0.78 & 0.76 & 0.71 & 0.61 \\
    CW-T & \textbf{0.88} & 0.86 & 0.70 & 0.73 & 0.00 & \textbf{0.74} & 0.73 & 0.70 & 0.63 & 0.00 &  CW-U & \textbf{0.88} & 0.87 & 0.84 & 0.87 & 0.78 & 0.75 & 0.71 & 0.61 \\
    CW-U & \textbf{0.86} & \textbf{0.86} & 0.72 & 0.53 & 0.00 & 0.64 & \textbf{0.75} & 0.45 & 0.46 & 0.00 &  CW-T & 0.86 & \textbf{0.87} & 0.84 & \textbf{0.87} & 0.77 & 0.75 & 0.71 & 0.60 \\
    DDN-T & \textbf{0.90} & 0.89 & 0.74 & 0.76 & 0.00 & 0.65 & \textbf{0.74} & 0.66 & 0.52 & 0.00 &  DDN-U & \textbf{0.88} & 0.87 & 0.84 & 0.87 & 0.77 & 0.76 & 0.72 & 0.61 \\
    DDN-U & \textbf{0.90} & 0.89 & 0.59 & 0.64 & 0.00 & 0.71 & 0.75 & 0.53 & 0.43 & 0.00 & DDN-T & 0.88 & 0.87 & 0.84 & 0.87 & 0.77 & 0.74 & 0.71 & 0.60 \\
    \bottomrule
    \end{tabular}%
  \label{tab:end2end}%
\end{table*}%

%This method could also be bypassed with BPDA~\cite{DBLP:conf/icml/AthalyeC018} which approximates the gradient of the target network. %online update of training data consuming exorbitant time and computational resources which makes it difficult at ImageNet scale~\cite{scale17}. 2) Modifying model architectures~\cite{BuckmanRRG18, DhillonALBKKA18} typically means manipulating the model gradients to make it intractable at inference time for adversarial attacks or use sub networks like defensive distillation~\cite{DBLP:conf/sp/PapernotM0JS16}. These methods have also been proved to be ineffective~\cite{DBLP:conf/icml/AthalyeC018,DBLP:journals/corr/CarliniW16} {\color{red} due to .....} 3) Reconstruction of inputs~\cite{GuoRCM18} during inference time could remove input perturbations to some extent so that the input could be classified correctly. This method could also be bypassed with BPDA~\cite{DBLP:conf/icml/AthalyeC018} which approximates the gradient of the target network.


\begin{table}[t]\small
  \centering
  \caption{Robustness of detectors for transform attacks.}
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    \multicolumn{8}{c}{Fashion-MNIST} \\
    \midrule
    Targeted & \multicolumn{6}{c}{Detector Performance} & \multicolumn{1}{|c}{Classification} \\
\cline{2-7}    \multicolumn{1}{c|}{Detector} &  ORG & VG & GBP & IG & LRP & X-Det & {Success Rate}\\
    \midrule
    ORG & 0.98 & 0.60 & 0.41 & 0.63 & 0.65 & \textbf{0.39} & 0.10  \\
    VG & 0.59 & 0.64 & 0.34 & 0.58 & 0.57 & \textbf{0.33} & 0.11 \\
    GBP & 0.63 & 0.55 & 0.57 & 0.63 & 0.71 & \textbf{0.55} & 0.10 \\
    IG & 0.66 & 0.69 & 0.37 & 0.98 & 0.93 & \textbf{0.37} & 0.10  \\
    \toprule
    \multicolumn{8}{c}{CIFAR10}\\
    \midrule
    Targeted & \multicolumn{6}{c}{Detector Performance} & \multicolumn{1}{|c}{Attack} \\
\cline{2-7}    \multicolumn{1}{c|}{Detector} &  ORG & VG & GBP & IG & LRP & X-Det & Classifier \\
    \midrule
    ORG & 0.98 & 0.56 & 0.53 & 0.55 & 0.57 & \textbf{0.40} & 0.11  \\
    VG & 0.40 & 0.69 & 0.42 & 0.39 & 0.49 & \textbf{0.27} & 0.11 \\
    GBP & 0.47 & 0.50 & 0.63 & 0.51 & 0.57 & \textbf{0.26} & 0.11 \\
    IG & 0.38 & 0.60 & 0.60 & 0.98 & 0.63 & \textbf{0.28} & 0.10  \\
    \bottomrule
    \end{tabular}%
  \label{tab:robustness}%
\end{table}%



 which are five neural network-based adversarial example detectors. Each detector


with white-/black-/grey-box threat model and targeted/untargeted adversarial specificities. It outperforms all state-of-the-art baselines for both detection/classification accuracy and robustness.

%The deep neural network models are long criticized for the black-box problem since their deep network structures can not be directly understood by human intuitions. In the literature, researchers proposed many interpreters to open the black-box of deep neural networks. These interpreters are divided as having local interpretability and having global interpretability~\cite{guidotti2019survey}. A local interpreter provides the explanation for a given input of a classifier, and a global interpreter provides explanation for the whole classifier. In this work, we focus on local interpreters since our adversarial example defense task is in the sample level. The usual approaches to implement local interpreters include using interpretable non-linear models, such as decision-tree and rule sets, as mimic models~\cite{wu2018beyond}, using linear models as local approximation of neural networks~\cite{ribeiro2016should}, and sensitivity analysis of attributes~\cite{sundararajan2017axiomatic}. In this work, we adopt the last approach, \ie sensitivity analysis, as our interpreter implementations. As shown in the literature~\cite{etmann2019connection} and Sec.~\ref{sec:connection}, the sensitivity-analysis-based interpretation has close connection with adversarial attacks.


%interpretation models have been proposed to provide interpretability for blackbox DNNs %Interpretable AI devotes to open the ``black boxes'' of As reported by Ref.~\ref{etmann2019connection}, the interpretability


%\subsection{Adversarial Attacks for visual classification}
%
%Previous research on finding adversarial examples assume attackers have full access to the models called ``white box" attacks. Many widely applied attacks leverage gradient of the model to guide their search towards efficient perturbations~\cite{carlini2017cw,bim,fgsm,su2019onepixel,moosavi2016deepfool,rony2019ddn,madry2017pgd}. In a more realistic setting, direct access to the target model is not always available to attackers. Thus, subsequent work also focuses on ``black box" attacks~\cite{papernot2016transferability,papernot2017practical,alzantot2019genattack,pmlr-v97-guo19a}. From an optimization perspective, to search for a suitable adversarial perturbation is to solve a certain object function with constrained noise payload under some measures like $L_0, L_2, L_\infty$.

%It has been discovered that there are some connections between DL model's interpretability and robustness to adversarial examples; for example, the local interpretations of images can also be adversarial attacked~\cite{underfire} and a more robust neural network has more interpretability~\cite{etmann2019connection}.  Nevertheless, we still can not directly use these connections to build a robust DL system that can be against defender-targeted adversarial attacks.

Although it has been discovered that there are some connections between interpretability and robustness of model to adversarial examples, such as the local interpretations of images can also be adversarial attacked~\cite{underfire} and a more robust neural network have more interpretability~\cite{etmann2019connection}, we still can not directly use these connections to build a robust DL system that can be against defender-targeted adversarial attacks.



%This finding inspired us to design a interpreter-guided adversarial detector and a rectifier.

adversarial examples detector and and rectifier guided by interpreter's outputs.

Following this line, we proposed as detector-rectifier combined adversary defense framework,

%\newpage

% lets our detector



%The %'s output as input. Here, we adopt four types of DL model interpreters to extract feature adversarial examples to train which adopts four types of DL model interpreters to generate feature of adversarial examples to train adversarial example detectors




%problem are not %adversarial training~\cite{}, modifying model architectures~\cite{}, rectifying adversarial examples %As reported by the literatures~\cite{}, %In this work, we focus on local interpreters since our adversarial example defense task is in the sample level. The usual approaches to implement local interpreters include using interpretable non-linear models, such as decision-tree and rule sets, as mimic models~\cite{wu2018beyond}, using linear models as local approximation of neural networks~\cite{ribeiro2016should}, and sensitivity analysis of attributes~\cite{sundararajan2017axiomatic}.


%, especially those data generated by strong $L_2$ adversaries like Deepfool~\cite{moosavi2016deepfool}, C\&W~\cite{carlini2017cw} and DDN~\cite{rony2019ddn}, which confirms our analysis.




%\input{sec-intro}
%\input{sec-rel}
%\input{sec-def}
%\input{sec-method}
%\input{sec-exp}
%\input{sec-con}



In other words, the model has seen all types of attack examples in the training step. This is very like letting immune systems generate antibodies by injecting the vaccine, so we call this setup as vaccinated training.

For each threat model, we consider two types of conditions for the detector training:
\begin{itemize}
  \item {\bf Vaccinated training:} Given an attacking model, we name it as ``vaccine'' attacker. The training samples of detector in vaccinated training contain adversarial examples generated by the vaccine attacker.
  \item {\bf Unvaccinated training:} In unvaccinated training, the training samples of detector don't contain adversarial examples generated by the vaccine attacker.
\end{itemize}
Vaccinated training likes letting immune systems generate antibodies by injecting the vaccine. Therefore, we use ``vaccinated'' and ``unvaccinated'' to name these two types of training conditions for detectors.

%of our \name model.
%${N}(\sigma, \mu)$, where $\sigma, \mu$ are set as the mean and standard deviation of pixels in $\bm{X}$.% \in [0,255], x_{ran} \in \mathbb{N}$. $x_{ran}$

%This is due to the inputs RF in \dname contains some sub-detectors of which the performance is not as better as the

%most of rows of the table, there are at least two or three of the sub-detectors have better performance than the baselines. This result evaluated the effectiveness of our idea that using interpretation map as features to detect adversarial examples.



%\begin{itemize}
%  \item The performance of \dname is superior to the three baselines, \ie PD, TWS, MHL. This result evaluated the effectiveness of our detector.
%  \item For every row of the table, there are at least two or three of the sub-detectors have better performance than the baselines. This result evaluated the effectiveness of our idea that using interpretation map as features to detect adversarial examples.
%  \item The detection performance of all detectors over CIFAR-10 is generally better than over Fashion-MNIST. CIFAR-10 is a more complex data set compared with Fashion-MNIST since it is a color image set while Fashion-MNIST is a grayscale one. As the table shows, X-Det has larger performance gains over the CIFAR-10 data set compared with over the Fashion-MNIST data set. This indicates our model has more significant advantages to the baselines over a more challenging scenario.
%  \item
%\end{itemize}

%the vaccine attacker. that is trained using adversarial examples generated by the


In the experiments,

the attacker generate adversarial examples using two threat models:
\begin{itemize}
  \item {\bf White-box attack} assumes attackers have knowledge of the network structure and parameters of the target classifier.
  \item {\bf Black-box attack} assumes attackers have no access to the model of the target classifier.
\end{itemize}
%, and use the
%\begin{itemize}
%  \item {\bf White-box attack} assumes attackers have knowledge of the network structure and parameters of the target classifier.
%  \item {\bf Black-box attack} assumes attackers have no access to the model of the target classifier.
%\end{itemize}


%Compared with the original image classifier $F$, the rectifier $F_{rec}$ is more robust to adversarial examples. However, its performance for benign examples is a little worse than $f$ due to some image information in $\mathcal{X}_{ran}$ were erased by the randomization. In order to combine the advantages of both $f$ and $f_{rec}$. We only use the rectifier to classify the adversarial examples picked out by the detector, and still handle benign examples with the original classifier.


\section{Rectifier}


Given an adversarial example $\bm{X}'$ with a predicted label $l$, our rectifier select a pixel as a suspect when its $\left|g_{ijl}\right|$ is larger than a threshold as
\begin{equation}\label{eq:masking_rate}
    \left|g_{ijl}\right| > \alpha \cdot \Big(g_{max}- g_{min}\Big) + g_{min},
\end{equation}
where $g_{max}$ and $g_{min}$ are the maximum and minimum values of pixel's $\left|g_{ijl}\right|$ in the adversarial example, and $\alpha$ is a perset parameter to control the ratio of suspect pixels.

For a suspect pixel, \name randomly disables it using two random numbers $x_{ran}$ and $u_{ran}$ as
\begin{equation}\label{}\small
    x_{a,b} : = \left\{\begin{aligned}
  & x_{a,b} &~~~ \mathrm{if}~~ u_{ran} = 0 \\
  & x_{ran} &~~~ \mathrm{if}~~ u_{ran} = 1
\end{aligned}\right.,
\end{equation}
where $u_{ran}\in \{0,1\}$ follows a Bernoulli distribution. If $u_{ran} = 0$, we keep $x_{a,b}$ as its raw value, otherwise we set it as a random value $x_{ran} \in [0,255], x_{ran} \in \mathbb{N}$. $x_{ran}$ follows a normal distribution ${N}(\sigma, \mu)$, where $\sigma, \mu$ are set as the mean and standard deviation of pixels in $\bm{X}$.

%guided by their InSen, the attack effects of adversarial examples might be dampened. {\bf Insight III:} As mentioned in Sec.~\ref{sec:motivation}, the $L_2$ norms of input sensitivity for adversarial examples are significant larger than benign examples. Thus, the pixels with large input sensitivity $\left|\partial \mathcal{L}/\partial x_i\right|$ are very likely to have been modified by the attack algorithm. Therefore, we conjecture if we remove the polluted pixels guided by their InSen, the attack effects of adversarial examples might be dampened.

%%%Jimmy
Given an adversarial example $\bm{X}'$ with a predicted label $l$, the rectifier calculates a mask matrix $\bm{M} \in \mathbb{R}^{I\times J}$ to pick the large $\left|g_{ijl}\right|$ pixels out as
\begin{equation}\label{eq:mask}
    m_{ij} = \left\{\begin{aligned}
  & 1 &~~~ \mathrm{if}~~ \left|g_{ijl}\right|  \ge \alpha \cdot (g_{max}- g_{min}) + g_{min} \\
  & 0 &~~~ \mathrm{if}~~ \left|g_{ijl}\right|  < \alpha \cdot (g_{max}- g_{min}) + g_{min}
\end{aligned}\right.
\end{equation}
where $m_{ij}$ is the item of $\bm{M}$, $g_{max}$ and $g_{min}$ are the maximum and minimum $\left|g_{ijl}\right|$ values in $\bm{X}'$, and $\alpha$ is a preset parameter to control the ratio of pixels to be altered. Then, we use $\bm{M}$ to rectify the adversarial example $\bm{X}'$ as
\begin{equation}\label{eq:rectifier}
    \bm{X}^{(r)} = Ret(\bm{X}') = \mathrm{clip}_{[0,255]}\left(\delta \bm{M} \odot  \bm{X} \right),
\end{equation}
where $\odot$ is a Hadamard product of matrices, and the random number $\delta$ follows a normal distribution $N(0, \sigma)$ of which $\sigma$ is set as the standard deviation of pixels in $X_a$.  $\mathrm{clip}_{[0,255]}(\cdot)$ is a function to maintain $\bm{X}^{(r)}$ into $[0,255]$.


%Notice that we only try Vallina Gradients[] to interpret the detector in this paper for simplicity. We believe that other interpreting methods also work.

%For an adversarial example, its prediction label $l$ is unreliable. Since the pixels with large $\left|g_{ijl}\right|$ play important role in the unreliable label generation, the information offered by the pixels with large  $\left|g_{ijl}\right|$ are also unreliable. These pixels are very likely to have been modified by attackers. Therefore, we argue that removing the polluted pixels that are indicated by $\left|g_{ijl}\right|$ can weaken the attack effects of adversarial examples.

%importat large $\left|g_{ijl}\right|$

%When the ratio of removed pixels increases, the success rate increases again. The reason is too many zero pixels may reduce the accuracy of the classifier. This requires us to design an elaborate approach to pick out the polluted pixels. Based on the phenomenon revealed by Tab.~\ref{tab:toy_exp}, we proposed our rectifier model.

%We define an adversarial example that is detected by the detector as a matrix $\bm{X}$, where the element $x_{a,b}$ is the pixel at the location $(a,b)$~\footnote{For the sake of discussion, we use the signal channel image as an example to introduce our rectifier.}.

calculate an index for each pixel $x_{ij}$ as
\begin{equation}\label{}
  s_{ij} = \left| ~g_{ijl} \frac{\partial \mathcal{L}\big(F(X'), l\big)}{\partial F(X')}~\right|.
\end{equation}
Here, the gradients of the loss function $\mathcal{L}$ is introduced to in


rectifier erase the adversarial perturbation by altering those potential pixels. A mask $M$ is defined as:
\begin{equation}\label{eq:mask}
    M_i = \left\{\begin{aligned}
  & 1 &~~~ \mathrm{if}~~ S_i  \ge \alpha \cdot (S_{max}- S_{min}) + S_{min} \\
  & 0 &~~~ \mathrm{if}~~ S_i  < \alpha \cdot (S_{max}- S_{min}) + S_{min}
\end{aligned}\right.
\end{equation}

with a certain type of interpretation inputs, the example usually cannot fool the sub-detector with other types of interpretation inputs.

target classifier gives the prediction label mainly

%Therefore, we argue that removing the polluted pixels that are indicated by $\left|g_{ijl}\right|$ can weaken the attack effects of adversarial examples.


 Since the pixels with large $\left|g_{ijl}\right|$ play important role in the unreliable label generation, the information offered by the pixels with large  $\left|g_{ijl}\right|$ are also unreliable.


In adversarial example, the large $\left|g_{ijl}\right|$ pixels play an important role to generate an unreliable prediction $l$,

For an adversarial example with an unreliable prediction class $l$, the information offered by the pixels with large  $\left|g_{ijl}\right|$ are also unreliable.

some one can designed a model to attack one type of interpretation of


We combine

It is tough to generate an adversarial example that can keep its interpretation be similar to its benign counterpart's interpretation for two types of interpretation methods at the same time. Therefore, the ensemble detection approach adopted by \name is much more robust than a signal detector.

%We use the training data set to train the sub-detectors and the ensemble detector. , such as FGSM~\cite{fgsm} and Deepfool~\cite{moosavi2016deepfool}, while $\mathcal{X}'_{L_\infty}$ are generated by $L_\infty$ attackers, such as PGD~\cite{madry2017pgd}, CW~\cite{carlini2017cw} and DDN~\cite{rony2019ddn}. We mix $\mathcal{X}^\circ$, $\mathcal{X}'_{L_0}$, and $\mathcal{X}'_{L_\infty}$ as a training data set.For each example in the training data set, there is label vector $\hat{\bm{z}} \in \{0,1\}^3$, where $\hat{\bm{z}} = (1,0,0)$ is for clean examples, $\hat{\bm{z}} = (0,1,0)$ is for $L_0$ attacks, and $\hat{\bm{z}} = (0,0,1)$ is for $L_\infty$ attacks. We use the training data set to train the sub-detectors and the ensemble detector.

%There are two ways to train a sub-detector. The first way is for each %The training of sub-detectors have two issues. The first %The outputs $\bm{z}$ in Eq.~\eqref{eq:detector_inter} and Eq.~\eqref{eq:detector_org} are one-hot vectors for multiple classification. In order to enhance generalization of sub-detectors, we classify input examples as three categories: clean (benign example), $L_2$ attacks, and $L_\infty$ attacks. Given a set of clean examples ${X}$, we use different adversarial attack methods to generate two sets of adversarial examples as ${X}'$ and  ${X}''$, where $\mathcal{X}'$ are generated by $L_2$ attackers, such as FGSM~\cite{fgsm}, Deepfool~\cite{moosavi2016deepfool}, and $\mathcal{X}''$ are generated by $L_\infty$ attackers, such as PGD~\cite{madry2017pgd}, CW~\cite{carlini2017cw} and DDN~\cite{rony2019ddn}. We use these data to train a

%\subsubsection{Sub-Detector Training}
%
%Given a set of benign examples $\mathcal{X} = \{\bm{X}^\circ_1, \ldots, \bm{X}^\circ_N\}$, a target classifier $F$, and an adversarial attack method $A$, we can generate a set of adversarial counterparts of $\mathcal{X}$ as $\mathcal{X}' = \{\bm{X}'_1, \ldots, \bm{X}'_N\}$. Then, we mix $X$ and $X'$ as training data set as
%\begin{equation}\label{}%\small
%  \mathcal{X} = \Big\{\left(\bm{X}^\circ_1, \bm{z}_1\right), \ldots, \left(\bm{X}^\circ_N, \bm{z}_N\right), \left(\bm{X}'_1, \bm{z}'_1\right), \ldots, \left(\bm{X}'_N, \bm{z}'_N\right)\Big\},
%\end{equation}
%where $\bm{z} = (z^+, z^-)$ is a one-hot coding of benign/adversarial label. $\bm{z}_n = (1,0)$ for benign examples and $\bm{l}'_n = (0,1)$ for adversarial examples.


%The simplest training method for sub-detectors is using a

In computer science and statistics community, XAI studies include designing high performance transparent ``white-box'' models, such deep Bayesian networks, and opening ``black-box'' of the models that cannot be directly understood by human intuition, such as deep learning interpretation. Obviously, our approach belongs to the second class.

\begin{equation}\label{eq:attacker_update}
  \bm{X}^{(i+1)} = \Pi_{B_\varepsilon(\bm{X}_\circ)}\left(\bm{X}^{(i+1)} - \alpha \frac{\partial \ell\left(F(X),~~ \bm{y}_{T}\right)}{\partial X}\Bigg|_{X=X^{(i-1)}}\right),
\end{equation}

\end{equation}
\begin{equation}\label{eq:attacker_update}
  \bm{X}^{(i+1)} := \Pi_{B_\varepsilon(\bm{X}_\circ)}\left(\bm{X}^{(i+1)} - \alpha \frac{\partial \mathcal{L}}{\partial F} \frac{\partial F(\bm{X}^{(i)})}{\partial \bm{X}^{(i)}}\right),
\end{equation}

%The baseline $x'$ can be any image but integrated gradient usually uses a blank picture as the baseline.

%along the $i^{th}$ dimension for an input $x$ and baseline $x'$ is defined as the follow:




%$$ IntGrad_i = (x_i-x'_i)\times \int_{\alpha=0}^{1} \frac{\partial F(x'+\alpha\times(x-x'))}{\partial x_i}\, d\alpha$$

\section{Motivation}~\label{sec:motivation}




%\section{The Basic Idea}

In this section, we will briefly introduce our motivation and the inherent idea of our method.

\begin{myDef}[Adversarial Sample]
    For a benign input $\bm{x}$ and its predicted label $\hat{\bm{y}}$ in the classifier $f$,
    we define its adversarial counterpart as $(\bm{x}',\hat{\bm{y}}')$, where $\|\bm{x} - \bm{x}'\|_2 < \epsilon$  and  $\hat{\bm{y}} \neq \hat{\bm{y}}'$.
\end{myDef}

\begin{myDef}[Input Sensitivity (InSen)]
    For an input $\bm{x}$ and its predicted label $\hat{\bm{y}}$, we define its input sensitivity as
    \begin{equation}~\label{eq:InSen}
        S(\bm{x},\hat{\bm{y}}) = \left | \frac{\partial \mathcal{L}(\bm{x}, \hat{\bm{y}})}{\partial \bm{x}} \right |,
    \end{equation}
    where $\mathcal{L}(\cdot)$ is the cross entropy loss function of $f$.
\end{myDef}

Since most of the adversarial attacks use network gradient of input images as a  guide to search perturbations~\cite{moosavi2016deepfool,carlini2017cw,rony2019ddn}, {\em the input sensitivity, which
is a form of gradient, of a benign sample and its adversarial counterpart usually have significant difference}. The basic idea of our method is using InSen as features to design adversarial sample detectors. In order to prove our idea, we give following analysis.


For the sake of discussion, we decompose the classifier $f$ as three parts:

1) The first part is a function that maps an input $\bm{x}$ into a representation vector $\bm{z}$, which is denoted as $\bm{z} = g(\bm{x})$.

2) The second part is a fully connection (FC) layer to calculate the prediction indexes of each classes. For the $i$-th class, the FC layer calculates an index $a_i = \bm{w}_i^\top \cdot \bm{z}$.

3) The third part is a softmax function to calculate the prediction probability of each class, which is denoted as $\bm{\hat{y}} = \sigma(\bm{a})$. For class $i$, this part is in the form of
\begin{equation}
    \hat{y}_i = \frac{\exp(a_i)}{\sum_{j=1}^N\exp(a_j)}, i \in \{1, \ldots, L\}.
\end{equation}
%\end{enumerate}
In other words, the classifier $f$ is in the form of
\begin{equation}
    \hat{y}_i = f_i\left(\bm{x}\right) = \sigma\left(\bm{w}_i \cdot g\left(\bm{x}\right)\right),~~i \in \{1, \ldots, L\}.
\end{equation}


Given two classes $m,n$, the label of the sample $\bm{x}$ with  $\bm{z}= g(\bm{x})$ is decided by the hyperplane as
\begin{equation}
    (\bm{w}_m - \bm{w}_n)^\top \cdot \bm{z} = 0.
\end{equation}
We define a generalized distance of the sample $\bm{x}$ to the classification hyperplane as
\begin{align}\label{eq:dist_z}
    {Dist}_z\left(\bm{x}\right) = \frac{\left|(\bm{w}_m - \bm{w}_n)^\top \cdot g(\bm{x})\right|}{\left\|\bm{w}_m - \bm{w}_n\right\|_2}.
\end{align}


For the sample $\bm{x}$ with the predicted class $m$, its input sensitivity is in the form of
\begin{equation}\label{General Case Gradient}\small
    \begin{aligned}
        S(\bm{x}, \bm{\hat{y}}) &=\Bigg|\sum_{p\neq m,n}{\frac{C_2}{\sum_{q}\exp{\left(a_q-a_p\right)}} } \\
         &+{\frac{C_1}{\exp{\underbrace{\left(\left(\bm{w}_m-\bm{w}_n\right)^\top\bm{z}\right)}_{\mathrm{Term~I}}} + \sum_{q \neq m}\exp{\left(a_q-a_n\right)}}}\Bigg|,
    \end{aligned}
\end{equation}
where $C_1  =  \left(\frac{\partial a_n}{\partial \bm{x}}-\frac{\partial a_m}{\partial \bm{x}} \right)$ and $C_2  =  \left(\frac{\partial a_p}{\partial \bm{x}}-\frac{\partial a_m}{\partial \bm{x}} \right)$. Since the predicted label of $\bm{x}$ is $m$, $a_m > a_n$ and $(\bm{w}_m-\bm{w}_n)^\top\bm{z}>0$. Therefore, the {\em Term I} in Eq.~\eqref{General Case Gradient} is in direct proportion to ${Dist}_z (\bm{x})$. In other words, the InSen $S(\bm{x})$ of an example has an increasing trend when its generalized distance to the classification hyperplane decreases, \ie ${Dist}_z\left(\bm{x}\right)$ decrease. Therefore, we get following insights:

{\bf Insight I:}{ The samples with closer distances to the classification hyperplane usually have lager input sensitivities}.

{\bf Insight II:}{ For many adversarial attack methods~\cite{moosavi2016deepfool,carlini2017cw,rony2019ddn}, the optimization object restricts size of the perturbations (such as restricting L2 metric of perturbations). Therefore, their adversarial examples are very likely just to cross the decision boundary. Thus, their input sensitivity should be bigger than normal input of that class due to a small $Dist_z$.}

%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.3]{pics/norm/scatter_mnist_gradient_L2norm.png}
%    \caption{$L_2$ norm of InSen for adversarial examples over MNIST.}
%    \label{pic:mn_grad_l2}
%\end{figure}

%\begin{figure}[t]
%    \centering
%    \includegraphics[scale=0.24]{L2attack_norm.pdf}
%    \caption{$L_2$ norm of InSen for clean and adversarial examples. Left: MNIST; Right: CIFAR-10.}
%    \label{pic:mn_grad_l2}
%\end{figure}


Fig.~\ref{pic:mn_grad_l2} illustrates the $L_2$ norms of InSen for clean and malicious inputs from MNIST and CIFAR-10 (setups see the experiment section). The InSen size of clean data are very tiny, while that of the malicious data are quite gigantic. This empirical result confirmed our Insights. We can use the InSen as a feature to detect adversarial samples.


%, especially those data generated by strong $L_2$ adversaries like Deepfool~\cite{moosavi2016deepfool}, C\&W~\cite{carlini2017cw} and DDN~\cite{rony2019ddn}, which confirms our analysis.
%In the experiments, we divide an image set as a training set and a test set. For the two sets, we use an attacker to generate their respective adversarial samples and construct adversarial/benign samples mixed training and test sets. The new training and test sets are respectively adopted to train and test the performance of our detector and baselines. counterparts, and mix the training samples and adversarial counterparts as an adversarial/benign classification training set, namely A-B training set. adversarial samples for a classifier $F$ over the training samples, and mix these adversarial samples with an equal number of benign training samples to construct an adversarial/benign classification training set, namely A/B training set. We use The experiment adopts an attacker $D$ to generate adversarial samples for a classifier $F$, and then mix these adversarial sample with an equal number of benign samples as adversarial/benign classification data set.
%We use the detector to classify these adversarial/benign samples to evaluate the performance of our detector.
%and evaluate the performance of our detector and baselines over the test adversarial and original samples.


%We consider two conditions for detection performance evaluation, namely {\em vaccinated} and  {\em unvaccinated}.
%In the vaccinated condition, the detector has been trained by the adversarial samples that are generated by the attacker model in the training set.
%unvaccinated %attack method %use a detector $Det$ to detect %The adversarial attacks

Classical


the items that have the closest connection with adversarial attacks  $g_{::l}$

In the sub-detectors, the inputs are the slice of the tensor $\mathcal{\bm{G}}$ corresponding to

In our implementations, the CNN networks are VGG11 networks~\cite{vgg11}.

where $l$ is the class predicted by the $F(\bm{X})$.


Interesting, a similar principle is also adopted by designing of attackers. Using the PGD~\cite{PGD} attacker as an example, given a benign input $\bm{X}$, PGD perturbs the pixel $x_{ij}$ to fool a classifier $F$ to given an output $l_a$ as
\begin{equation}\label{eq:attacker_update}
  {x}_{ij}^{(\tau+1)} := \Pi_{B_\varepsilon(\bm{X}_\circ)}\underbrace{\left[{x}_{ij}^{(\tau)} - \alpha \frac{\partial  \mathcal{L}\left(F\left(\bm{X}^{(\tau)}\right),~~ l_a\right)}{\partial {x}_{ij}^{(\tau)}}\right]}_{\mathrm{Term~I}},
\end{equation}


%In the literatures, there are several different technical routs to implement a local interpreter~\cite{??}.


In our \name model, interpretations of target classifiers are adopted to detect adversarial examples.



indicates the real object of the image, for example a dog in the image.

%signification interpretation matrix $\bm{G}$ for adversarial samples


%In this way, we could design a model to


%Typically, an adversarial input is generated by modifying a benign input via pixel perturbation. Given a benign input $\bm{X}$, attackers adopt a project gradient descent on the loss function of $F$ to perturb the input as
%\begin{equation}\label{eq:attacker_update}
%\begin{aligned}
%  \bm{X}^{(i+1)} &:= \Pi_{B_\varepsilon(\bm{X}_\circ)}\left(\bm{X}^{(i+1)} - \alpha \frac{\partial  \mathcal{L}\left(F(\bm{X}^{(i)}),~~ \bm{y}_{T}\right)}{\partial \bm{X}^{(i)}}\right)\\
%                 &= \Pi_{B_\varepsilon(\bm{X}_\circ)}\left(\bm{X}^{(i+1)} - \alpha \frac{\partial \mathcal{L}}{\partial F} \frac{\partial F(\bm{X}^{(i)})}{\partial \bm{X}^{(i)}}\right),
%\end{aligned}
%\end{equation}
%where $\Pi_{B_\varepsilon(\bm{X}_\circ)}$ is the projection operator to limit  $\mathrm{Dist}(\bm{X}_a,\bm{X}_\circ) < \varepsilon$, $\ell$ is the loss function of $F$, and $\bm{y}_{T}$ is the true label of $\bm{X}$.

%As Eq.~\eqref{eq:attacker_update} shows, the adversarial sample generation usually focus on restrain overall perturbation using the projection operator $\Pi_{B_\varepsilon(\bm{X}_\circ)}$. However, the size of ${\partial \ell(F(\bm{X}),\bm{y}_{T})}/{\partial \bm{X}}$ in Eq.~\eqref{eq:attacker_update} is not restrained by any mechanism. In Eq.~\eqref{eq:attacker_update}, the pixel with large $\partial \ell / \partial x_{ij}$ have higher perturbation than with the lows. In this way, the value of $\partial \ell / \partial x_{ij}$ for all image pixels may occur large change. This means that the pixels having large influences to loss function $\ell$ are significantly perturbed by an attacker.

%An adversarial sample generator modifies $\bm{X}$ through move $x_{ij}$ toward to a direction of $\partial \ell / \partial x_{ij}$ is larger than other of $\bm{X}$ on the original domain, but for the $\ell(F(\bm{X}),\bm{y}_{T})$ domain,

%the common approach adopted by adversarial sample generator

%Intuitively, we can see Eq.~\eqref{eq:attacker_update}




